Lattice Dynamics of Energy Materials Investigated by Neutron Scattering

In this thesis, I discuss several basic science studies in the field of energy materials using neutron scattering as a probe for the lattice dynamics. To enable understanding of neutron scattering spectra, I also use computational and theoretical methods. These methods and neutron scattering in general are discussed in detail in Chapter 2. It is assumed that the reader is familiar with basic quantum mechanics as well as with solid state physics topics including the band theory of electrons, harmonic lattice dynamics, and molecular dynamics. For the unfamiliar reader, the details of electronic structure theory and lattice dynamics that are needed to understand the methods in Chapter 2 are provided in Chapters 3 and 4. In the remaining chapters, these methods are applied to the study of several energy materials: cuprate La2CuO4,(hybrid) solar perovskite CH3NH3PbI3, and thermoelectric clathrate Ba8Ga16Ge30.

==> flashed_rutile/flashed_rutile.tex <==

\chapter{Electric-current induced modifications of rutile TiO$_2$}
\label{chp:flashed_rutile}


\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{flashed_rutile/graphical_abstract.png}
    %\caption{}
\end{figure*}

In-situ diffuse neutron scattering experiments revealed that when electric current is passed through single crystals of rutile TiO$_2$ under conditions conducive to flash sintering, it induces the formation of parallel planes of oxygen vacancies. Specifically, a current perpendicular to the $c$-axis generates planes normal to the (132) reciprocal lattice vector, whereas currents aligned with the $c$-axis form planes normal to the (132) and to the (225) vector. The concentration of defects increases with incresing current. The structural modifications are linked to the appearance of signatures of interacting Ti$^{3+}$ moments in magnetic susceptibility, signifying a structural collapse around the vacancy planes. Electrical conductivity measurements of the modified material reveal several electronic transitions between semiconducting states (via a metal-like intermediate state) with the smallest gap being 27 meV. Pristine TiO$_2$ can be restored by heating followed by slow cooling in air. Our work suggests a novel paradigm for achieving switching of electrical conductivity related to the flash phenomenon.

\section{Structural and electronic transformations in TiO$_2$ induced by electric current}

\begin{comment}
\author[1]{Tyler C. Sterling\corref{cor}}
\ead{ty.sterling@colorado.edu}
\author[2]{Feng Ye}
\author[3]{Seohyeon Jo}
\author[1]{Anish Parulekar}
\author[1]{Yu Zhang}
\author[1,4]{Gang Cao}
\author[5]{Rishi Raj}
\author[1,4]{Dmitry Reznik\corref{cor}}
\ead{dmitry.reznik@colorado.edu}
\cortext[cor]{Corresponding Author}

\affiliation[1]{organization={Department of Physics, University of Colorado Boulder}, city={Boulder}, postcode={80309}, state={Colorado}, country={USA}}
\affiliation[2]{organization={Neutron Scattering Division, Oak Ridge National Lab}, city{Oak Ridge}, postcode={37830}, state={Tennessee}, country={USA}}
\affiliation[3]{organization={Materials Science and Engineering, University of Colorado Boulder}, city={Boulder}, postcode={80309}, state={Colorado}, country={USA}}
\affiliation[4]{organization={Center for Experiments on Quantum Materials, University of Colorado Boulder}, city={Boulder}, postcode={80309}, state={Colorado}, country={USA}}
\affiliation[5]{organization={Department of Mechanical Engineering, University of Colorado Boulder}, city={Boulder}, postcode={80309}, state={Colorado}, country={USA}}
\end{comment}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{flashed_rutile/main_fig.pdf}
    \caption{(a) Schematic of the in-situ neutron scattering flash experiment during the constant-current conditions in the typical I-V curve during flash in (b). When the E-field is increased to a critical value, the resistivity drops sharply ($\sim$ an order of magnitude); this occurs at about 7.5 minutes. (c) Scattering pattern from pristine (left) and flashed (right) samples in the $H$-$L$ plane with $K=0$. (d). Diffuse scattering features from the S1 dataset in (c) translated into the 1$^{st}$ Brillouin zone and summed as discussed in the text. (e) A model of a Magn\'eli phase shear plane as described in ref. \cite{bursill1971crystal}. The vector $\bm{q}^*$ in (d) and (e) points along $(1\bar{3}2)$ and the displacement vector for the shear in (e) is $1/2[011]$. (f) A model of the defect region in (e) showing different views (left) and an exploded view (right). The shear plane consists of chains of face-sharing octahedra (gray) separated by rutile-like edge sharing octahedra (blue). Between shear planes, the structure is rutile.}
    \label{fig:main_fig}
\end{figure*}

Flash sintering has emerged as a transformative technique for material processing, revolutionizing the synthesis and densification of ceramic materials \cite{yadav2023room,raj2021flash,raj2016analysis,raj2012joule,cologna2010flash}. This method involves the application of an electric field to significantly reduce the sintering time and temperature, achieving results comparable to traditional methods in mere seconds. This not only conserves energy but also paves the way for the creation of materials with novel properties.

In this study, we applied an electric field to rutile TiO$_2$ single crystals under flash sintering conditions, rapidly modifying the atomic structure and switching electrical resistivity from a high to low resistance state with novel temperature dependence. Our in-situ neutron diffuse scattering measurements reveal that this process consistently generates oriented parallel planes of structural defects, likely oxygen vacancies, which remain stable at room temperature. This altered form of TiO$_2$ shows several electronic transitions as a function of temperature and, at room temperature, exhibits a bandgap reduced from $\sim 3.05$ eV \cite{cronemeyer1952electrical,amtout1995optical} in the pristine material to 27 meV. Additionally, magnetic susceptibility measurements indicate an enhanced non-Curie-Weiss magnetic susceptibility, consistent with the presence of Ti$^{3+}$ ions with interacting moments, suggesting a structural collapse around the planes of oxygen vacancies. The formation of interacting moments by electric current suggests flash can be used to induce novel electronic physics. These findings offer a promising pathway towards engineering new devices, such as memristors, through the current-induced introduction of defects in TiO$_2$, opening new avenues for advanced material applications.


\section{Methods}

To understand the structural modifications of materials during flash, we designed and built an apparatus for in-situ neutron scattering measurements under controlled E-field and high temperatures at the CORELLI diffractometer at the Spallation Neutron Source (SNS) at Oak Ridge National Laboratory. This instrument combines the high efficiency of white beam Laue diffraction with energy discrimination, allowing us to measure both elastic and total scattering in a single experiment over large volumes of reciprocal space. It also accesses large momentum transfer Q and high momentum resolution to distinguish diffuse signals from nearby Bragg peaks \cite{ye2018implementation}.

Elastic neutron scattering experiments were performed on rutile TiO$_2$ single crystals with current applied along the $b$- and $c$-axes. For current along the $b$-axis, we measured a crystal in-situ and a pre-flashed one ex-situ, which was quenched in LN2 after being flashed in air. The in-situ experiments were conducted at multiple temperatures and current densities to study the dependence of scattering on flash conditions. For current along the $c$-axis, we measured one sample and one current density, with additional measurements on the $c$-axis flashed sample ex-situ using a low-background close cycle refrigerator to characterize structural modifications. In this study, we focus primarily on two samples: sample-1 (S1), flashed in \emph{air} with current along the $b$-axis and then quenched, and sample-2 (S2), flashed in \emph{vacuum} at the SNS with current along the $c$-axis. The dimensions of all samples were $10\times3\times 1$ mm.

Refining the atomic coordinates via analysis of Bragg intensities results in significant uncertainty due to experimental conditions being optimized for diffuse scattering measurements. We will address structural refinement following planned additional measurements, which are beyond the scope of the current project.

Temperature dependence of electrical resistivity and magnetic susceptibility was measured on a pristine single crystal and on S2 using the Quantum Design MPMS system. S1 broke during the neutron scattering experiments, rendering the pieces too small for reliable transport measurements. The conductivity of the pristine sample was too low to measure, and the flashed sample was too thin to measure conductivity in the $ab$ plane. The sample environment at CORELLI does not support logging I-V data, so we performed an offline experiment to measure the I-V curve in fig. \ref{fig:main_fig}b on a different sample under similar flash conditions to emphasize the non-linear change in resistivity that is typical during flash experiments \cite{yadav2023room,raj2016analysis}. 




\section{Results}

During flash sintering \cite{raj2016analysis}, a sample is first held at an elevated temperature, and an electric field (E-field) is applied across it (fig.  \ref{fig:main_fig}a). The E-field is increased continuously or stepwise until the resistivity begins to fall nonlinearly, which in fig.  \ref{fig:main_fig}b occurs at 6 minutes when the E-field reaches 150 V/cm. Eventually, at around 8 minutes, the sample abruptly switches to a low-resistance state, and the power supply reaches the current limit. At this point, the voltage is automatically regulated to maintain constant current, signaling the onset of flash. Alternatively, a constant E-field can be applied, and the temperature increased to a critical value where the resistivity drop occurs. In the flash state, the sample usually glows brightly due to electroluminescence. This process exhibits some material-dependent variability; in some cases, flash occurs under moderate critical E-field strengths at room temperature. Furthermore, this glow might not always be visible, depending on the luminescence spectrum and brightness, which vary with material properties \cite{roy2023structural}.

Our experiments show that TiO$_2$ loses some oxygen during flash. Turning off the current and slowly cooling the sample in air often leads to re-absorption of oxygen, restoring the pristine high-resistance state. Remarkably, the sample remains in the flash state under steady-state current conditions, even if removed from the furnace. Immersing the flashing sample in liquid nitrogen (LN2) followed by shutting off the current, or conducting flash sintering in a vacuum, prevents oxygen re-absorption.

\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{flashed_rutile/combined_2.pdf}
    \caption{Volumetric plots of the summed S1 (a) and S2 (b) datasets. The dashed \textcolor{red}{red} lines label the (132) features, whereas black arrows label the (225) features. (a) Sample was flashed and quenched in air and the current was perpendicular to the $b$-axis. (b) The sample was flashed in vacuum and then was allowed to cool. Current was parallel to the $c$-axis. The artifact labeled in (b) is from neutrons saturating the detectors; it is not physically interesting.}
    \label{fig:summed_views}
\end{figure}

Our neutron scattering experiments provide significant insights into the structural transformations in TiO$_2$ under the influence of electrical current, with profound implications for understanding flash-induced modifications. We observed that Bragg peak positions consistently aligned with the tetragonal symmetry of the rutile structure across all datasets, indicating no symmetry breaking of the average structure upon the application of current. The primary changes induced by the Flash technique were confined to the local structure.

In this study, we focus primarily on two samples: sample-1 (S1), flashed in \emph{air} with current along the $b$-axis and then quenched, and sample-2 (S2), flashed in \emph{vacuum} at the SNS with current along the $c$-axis. We also discuss several in-situ measurements with current along the $b$-axis (see methods for details). The results of in-situ neutron scattering measurements with electrical current passing through the samples were qualitatively similar to those obtained from ex-situ flashed samples, with a notable difference for sample S2. Detailed results for the in-situ measurements at several temperatures and currents are provided in the supplementary information \cite{supp_info}. In the main text, we mainly focus on ex-situ measurements of samples S1 and S2 as quantitative analysis of the in-situ data was not possible due to the large furnace background.

As shown in fig.  \ref{fig:main_fig}, the primary effect of the flash process is the emergence of needle-like shoulders on the Bragg peaks, extending in all symmetry-equivalent (132) directions. Both S1 and S2 samples exhibited these (132) features; however, S2 also displayed less pronounced needles oriented along (225), as illustrated in fig. \ref{fig:summed_views}b. The differences in the apparent widths of features in fig.  \ref{fig:summed_views}a versus fig.  \ref{fig:summed_views}b are attributed to instrument resolution, as the two samples were mounted with different orientations in the scattering plane. In what follows, we use Miller indices in the basis of primitive rutile lattice vectors (tetragonal symmetry with $a=b\neq c$).

\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{flashed_rutile/combined_fig_5_and_7.pdf}
    \caption{Current and temperature dependence of the diffuse scattering features along different needles thru different Bragg peaks labeled in the figure. Background determined by taking cuts through nearby regions with no diffuse scattering was subtracted.  Sample ``$100^\circ$C post" is the in-situ flashed crystal after the field was turned off and the sample cooled back to the furnace temperature $100^\circ$C. Background due to the furnace and electrodes was subtracted. Since the needles aren't oriented along a high-symmetry direction, we plot data in $\textrm{\AA}^{-1}$. See the text and supp. info \cite{supp_info} for detailed explanation of the coordinates and orientation of the needles.}
    \label{fig:combined_line_cuts}
\end{figure}

The intensity and asymmetry of the needles varied from Bragg peak to Bragg peak due to structure factor effects. By projecting all diffuse scattering features into the first Brillouin zone, a sea urchin-like pattern emerged. We picked all Brillouin zones in each data set with significant diffuse scattering, translated these scattering intensities to the 1$^{st}$ Brillouin zone, then summed them (see fig.  \ref{fig:summed_views} and supp. info \cite{supp_info}). We call different symmetry-equivalent needles $k_{1}$, $k_2$, $...$, $h_1$, $...$, etc \cite{supp_info}. The sea-urchin structure is present for all currents and temperatures that we measured. The directions of the needles were determined by fitting the coordinates of their intersections with integrated planes of intensity cuts through the summed data. These needle directions are all equivalent under tetragonal symmetry operations. The direction of the needles is independent of current (see supp. info. \cite{supp_info}).

In fig. \ref{fig:combined_line_cuts}, we present current and temperature-dependent cuts along several different needles. These cuts are made along straight lines in reciprocal space that align with the needle orientations, rather than high-symmetry directions, and are presented in $\textrm{\AA}^{-1}$. Detailed fitting of the needle directions and additional cuts along needles are provided in the supplementary information \cite{supp_info}.

It is well-established that needle-like structures in diffraction correspond to planar correlations in real space. The primary effect of flash on TiO$_2$ is to produce either pancake-like clusters of defects and/or planar slip dislocations oriented perpendicular to the needles. Analysis of the S1 dataset, where we have the most comprehensive data, allowed us to estimate the correlation lengths of the defects to be approximately $46~\textrm{\AA}$ perpendicular to the pancake planes and $\sim200~\textrm{\AA}$ within the planes (line cuts perpendicular to the needles are resolution-limited: see supp. info \cite{supp_info}).

Figure \ref{fig:combined_line_cuts} compares the scattering intensity distribution for representative cuts along the needles of the in-situ sample at different electrical current densities and temperatures in the furnace. The pristine sample exhibited only resolution-limited Bragg peaks, with no diffuse scattering. In contrast, flashed samples displayed diffuse scattering tails on the Bragg peaks. Although needle orientation was independent of current (see supp. info. \cite{supp_info}), the diffuse intensity increased with higher current density. For identical sample volumes, which is the case for our experiments, an increase in diffuse scattering intensity corresponds to an increase in defect concentration. This increase was not linear; for example, 40 mA at 100C produced less diffuse intensity than higher currents, where the effect seemed to saturate. During the flash process, the sample temperature rises considerably due to heating by electric current and experiments to accurately characterize this heating are planned. Preliminary estimates based on Bragg peak intensities show that 500 mA results in extra heating of several hundred degrees ($^\circ$C). Despite this, the diffuse scattering pattern remains consistent with that of the post-flashed sample, which experienced no additional heating. This suggests that temperature does not significantly influence the diffuse scattering pattern.

The temperature dependence of the electrical conductivity of S2 (fig. \ref{fig:mat_props}b) at low temperatures $T \lesssim$ 50 K fits the semiconductor model $\sigma(T) = \sigma_0 \exp(-E_A/k_B T) $ with $E_A = $ 13.5 meV and $\sigma_0 = $ 39.7 (Ohm-cm)$^{-1}$. At high temperatures $T \gtrsim$ 150 K, $E_A = $ 15.2 meV and $\sigma_0 = $ 2.5 (Ohm-cm)$^{-1}$, although the fit is less precise. We estimate the band gap, $\Delta$, from $E_A = \Delta/2$. An alternative approach might involve assuming multiple gaps in the high-temperature regime \cite{yagi1996electronic,hasiguti1994electrical}.

In the intermediate temperature range (60 K $\lesssim T$ $\lesssim$ 150 K), the conductivity fits the model $\sigma(T) = 1/ [\rho_D + \rho_0 (T/\Theta)^n]$, consistent with metallic behavior. Here, $\rho_D$ represents the resistivity due to defect scattering, $\rho_0$ is the characteristic resistivity from other scattering forms, $\Theta$ is the temperature scale, and $n$ is the exponent. At low temperatures, $n = 5$ corresponds to electron-phonon scattering and $n = 2$ to electron-electron scattering, though $n = 1$ is often used empirically for small temperature changes. We fit $\rho_D,~\rho_0,$ and $n$. We find $\rho_D \approx$ 0 (Ohm-cm) an $n\approx 1$, so that $\sigma(T)\sim \sigma_0 \times (\Theta/T)$ with $\sigma_0 = 1/\rho_0 = $ 0.2 (Ohm-cm)$^{-1}$ and $\Theta =$ 654.5 K. Interestingly, $\Theta$ is similar to but lower than the known Debye temperature of pristine rutile TiO$_2$, $\Theta_D=$ 943 K \cite{wu1982elastic}, though the interpretation with $n\equiv 1$ is not physically meaningful. 

\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{flashed_rutile/materials_properties.pdf}
    \caption{Magnetic susceptibility $\chi$ (a), electrical conductivity $\sigma$ (b), and $1/\chi$ (c-d) of pristine and flashed S2 sample (see text). $\chi^f_{ab}$ and $\chi^f_c$ are the susceptibilities in the $ab$ plane and along the $c$-axis respectively. $\sigma^f_{c}$ is the conductivity along the $c$-axis of the flashed sample. The arrow indicates the position of the `dip' in the conductivity which coincides with anomalies in the susceptibility. The different curves plotted with $\sigma$ and $1/\chi$ corresponds to fits through different temperature regimes as discussed in the text. The gray markers in b) are conductivity data for TiO$_{1.9983}$ from ref. \cite{hasiguti1994electrical} divided by 10.}
    \label{fig:mat_props}
\end{figure}

The magnetic susceptibilities were analyzed assuming Curie-Weiss behavior to extract magnetic moments ($\mu_{eff} = \sqrt{8 C}$) and Curie-Weiss temperatures ($\Theta_{CW}$). A temperature-independent contribution ($\chi_0$) was also included in the susceptibility model: $\chi(T) = \chi_0 + C/(T-\Theta_{CW})$. Above approximately 60 K, the susceptibilities of the flashed sample deviated significantly from Curie-Weiss behavior (Figs. \ref{fig:mat_props}c-d). We separately fitted both the Curie-Weiss-like low-temperature regimes (dashed lines in Figs. \ref{fig:mat_props}c and d) and the full curves (dashed-dotted lines in Figs. \ref{fig:mat_props}c-d). Only the parameters extracted from the low-T regime for the flashed samples were physically sensible, and we focus on these here. Fits to the full temperature range are provided in the supplementary information\cite{supp_info}. As a reference, the pristine samples followed Curie-Weiss behavior up to $T\sim$300 K.

At low temperature for the flashed sample, $\mu_{eff} = 0.069~\mu_B$/Ti in the $ab$ plane and $\mu_{eff} = 0.065~\mu_B$/Ti along the $c$-axis for the flashed sample. The increase in the effective moment in S2 is consistent with the emergence of Ti$^{3+}$(3d$^1$) ions; the occurrence of Ti$^{3+}$ is typical of reduced rutile TiO$_2$ as shown before with x-ray photoelectron spectroscopy results from both electroformed TiO$_2$ \cite{szot2011tio2} and bulk reduced rutile Ti$_4$O$_7$ Magn\'eli phases \cite{kim2023performance,taguchi2010anomalous}. $\chi_0$ and $\Theta_{cw}$ are provided in the supp. info. \cite{supp_info}. In the pristine sample $\mu_{eff} = 0.024~\mu_B$/Ti in the $ab$ plane and $\mu_{eff} = 0.025~\mu_B$/Ti along the $c$-axis.

Both susceptibilities of the flashed sample show anomalies at $T \approx 165$ K (down-arrows in figs. \ref{fig:mat_props}b-d). Along the $c$-axis, there is a dip in the susceptibility; in the $ab$ plane, there is a ``kink". There are no corresponding anomalies in the susceptibilities of the pristine sample. Intriguingly, a minimum in the conductivity appears at the same temperature (\ref{fig:mat_props}b). There is also a maximum in the conductivity at $T\approx 60$ K (up-arrow in fig.  \ref{fig:mat_props}b); $T\approx 60$ L is where the susceptibilities of the flashed sample begin to deviate significantly from Curie-Weiss behavior (up-arrows in Figs. \ref{fig:mat_props}c-d). These findings reveal complex and nuanced changes in TiO$_2$ as a result of flash.



\section{Discussion and Conclusions}

Flash/quench treatment induces radical yet reproducible and potentially controlled modifications in atomic structure and bulk properties. In our study, we demonstrated that this treatment introduces planar defects into TiO$_2$, transitioning it to a low-resistance phase. Insulators, such as yttria-stabilized zirconia, often become metallic under similar conditions. In the quasi-2D quantum material Pr$_2$CuO$_4$, this treatment enhances oxygen vacancy ordering, thereby increasing the three-dimensionality of electrical resistivity and magnetization, and sharpening of Raman-active phonons \cite{roy2023structural}.

Despite the enigmatic nature of the atomistic mechanism behind flash, it has been successfully applied across a broad spectrum of materials, from metals like aluminum \cite{mcwilliams2018sintering,raj_private} and tungsten \cite{raj_private} to both simple and complex oxides \cite{raj2021flash}. Typically, ceramics requiring hours at approximately $\sim$1500$^\circ$C  to sinter can now be consolidated from powders in seconds at significantly lower temperatures under flash conditions. Recent advancements in flash sintering include synthesizing new materials, such as high-entropy oxides with exceptional lithium-ion conductivity for next-generation batteries \cite{yan2022reactive}, and transforming insulators into metals. Initially observed in polycrystalline materials and attributed to Joule heating at grain boundaries \cite{yu2017review}, flash sintering's discovery in single crystals \cite{yadav2017onset} revealed it as a bulk effect.

Rutile TiO$_2$, a wide-gap insulator transparent to visible light, becomes electrically conducting and light-absorbing when slightly reduced to TiO$_{2-x}$ ($x<2$) \cite{bursill1969new,hasiguti1970electrical,yagi1996electronic}.  This transformation is due to the formation of Magn\'eli phases, where oxygen vacancies aggregate into semiconducting planes, causing shear dislocation of adjacent rutile slabs \cite{bursill1969new, bursill1971aggregation, bursill1971crystal, bursill1970displacement, zhang2021andersson, liborio2008thermodynamics}. The chemical formulae of the Magn\'eli phases are Ti$_n$O$_{2n-1}$, with the orientation and density of defect planes depending on $n$. For commonly studied more-reduced phases ($4 \leq n \leq 10$), the shear planes are perpendicular to $(121)$ \cite{andersson1960crystal,zhang2021andersson}. For slightly-reduced phases, $15 \leq n \leq 39$, the shear planes are perpendicular to $(132)$ \cite{bursill1969new,bursill1971aggregation,chu1970new,yagi1977312}, with the displacement vector of the shear between adjacent rutile slabs being $1/2[0\bar{1}1]$ \cite{bursill1970displacement,yagi1996electronic}. These phases' two-dimensional character of the conducting planes containing Ti $3d$ electrons has the potential to host novel electronic properties \cite{taguchi2010anomalous,lechermann2017oxygen,watanabe2009raman,okamoto2004electronic,szot2011tio2}.

Our observations of needle-like structures forming along the (132) and equivalent crystallographic directions in both in-situ and quenched samples indicate the formation of the $(132)$ Magn\'eli phase. This structure is notoriously difficult to synthesize via conventional annealing, leaving many of its properties unexplored until now \cite{hasiguti1994electrical,hasiguti1970electrical,yagi1996electronic}. Our research bridges this knowledge gap, showing consistent formation of the (132) phase in both S1 and S2 samples despite varied preparation conditions and across a wide range of temperatures and current densities. In particular, the (132) scattering emerges as a dominant feature in the S2 sample, though subtler needle-like patterns along (225) also warrant mention. The relationship of this (225) feature to the current direction or vacuum environment in S2 remains an open question, which our ongoing research seeks to clarify. Additionally, we acknowledge the prior identification of disordered (101), (100), and (725) features in slightly reduced rutile \cite{bursill1969new,hasiguti1994electrical}, highlighting that while other defects do form, the (121) and (132) phases are the most pronounced. 

Besides studies using conventional reduction, our observation of oxygen defects due to electrical current is consistent with earlier work on flash sintered TiO$_2$ \cite{yoon2018measurement,li2019nanoscale,masuda2024optical,charalambous2018situ}. In particular, measurements of elastic properties of in-situ flashing rutile TiO$_2$ revealed anomalous softening which was attributed to the formation of oxygen defects. Under DC current, planar defects were observed \cite{li2019nanoscale} while under AC current, Magn\'eli phases were notably absent \cite{masuda2024optical} which emphasizes the fact that current has substantial impact on the nature of defect formation. Studies using in-situ x-ray diffraction found anomalous displacement of oxygen atoms \cite{yoon2018measurement} and peak splitting \cite{charalambous2018situ}. Large oxygen displacements are consistent with the formation of oxygen defects, while peak splitting is consistent with the formation of an enlarged unitcell containing oxygen defects (c.f. Magn\'eli phases, which have enlarged rutile-like unitcells).

Previous efforts to synthesize Magn\'eli phases through annealing required extensive periods, tens of hours or more at above 1000$^\circ$C, to achieve homogeneously reduced samples \cite{hasiguti1994electrical,hasiguti1970electrical,yagi1996electronic}. In contrast, our research demonstrates that the $(132)$ phase can be rapidly produced in bulk crystals in just minutes at significantly reduced temperatures, approximately 400°C, using flash sintering. This result raises intriguing questions about whether the $(121)$ phase could also be synthesized in single crystals exhibiting greater oxygen deficiency through flash sintering. The successful creation of this phase under such conditions has been documented in ceramic TiO$_2$ \cite{xue2023situ}. 

Comparing our findings with earlier research on slightly reduced rutile, which featured lower oxygen vacancy concentrations ($0.00001 < x < 0.0001$) \cite{yagi1996electronic,hasiguti1994electrical}, provides valuable insights. In these cases, shear planes were either absent or scarcely formed, with electrical transport primarily occurring through hopping between isolated Ti interstitials dispersed throughout the material. The emergence of a few shear planes at higher vacancy concentrations was found to impede hopping, leading to reduced conductivity. However, the pronounced scattering intensity related to the (132) shear planes in our neutron diffuse scattering data indicates a substantially higher $x$ in our samples, signifying a greater concentration of oxygen vacancies. Previous studies estimated activation energies to be around $\sim1$ meV and reported conductivity an order of magnitude higher than that observed in our samples, which possess notably larger oxygen vacancy concentrations. This discrepancy likely stems from the distinct nature of transport mechanisms: in earlier studies, shear planes primarily served to scatter carriers, whereas in our samples, transport appears to be predominantly confined within the planes themselves, akin to behavior seen in more significantly reduced Magnéli phases, such as Ti$_4$O$_7$ \cite{szot2011tio2}.

During flash, it is possible that only existing oxygen vacancies order due to the electric field, but more likely, new vacancies form with excess oxygen diffusing out of the sample and vacancies diffusing into the bulk \cite{bursill1972crystallographic,setvin2015aggregation}. The formation of bulk oxygen defects in rutile is already well known \cite{bursill1969new,bursill1971aggregation,cho2006first}, but it was only recently shown the formation of oxygen Frenkel defects, a precursor to isolated oxygen vacancies, is enhanced by electric fields \cite{abdelouahed2015relevance}. Under applied electric field, thermal displacements could promote the formation of oxygen defects, leading to enhanced conductivity (due to e.g. impurity levels) and the formation of currents and Joule heating, leading to the formation of even more defects and so on. It is also possible that the rapid heating experienced at the onset of flash, rather than the electric field itself, is responsible for the defects formation \cite{kermani2021ultrafast}, but this avenue of investigation is beyond the scope of this work. 

Before concluding, we mention that the formation of \emph{bulk} defects might be unique to rutile TiO$_2$, which is already known to form bulk oxygen defects (c.f. Ti$_4$O$_7$ Magn\'eli phases), even without electrical currents. In other oxides, defects might be localized near the surface; this is the subject of ongoing investigation.

We demonstrated that TiO$_2$ can transition from a high-resistance to a low-resistance state through the application of electric current (fig.  \ref{fig:main_fig}b), a change attributed to the formation of oxygen defect planes. The changes induced by current are persistent, but can be reversed by annealing in an oxygen rich environment. The concentration of defects can be controlled via the in-situ current density or by quenching in liquid nitrogen to freeze in defects. The defects are consistent with the formation of Magn\'eli phases in slightly reduced rutile; however, the temperature dependence of conductivity in flashed rutile TiO$_2$ shows several electronic phase transitions that are different from what has been previously observed. The anomalous electronic behaviour suggests that novel electronic physics can be induced by passing electric current through rutile TiO$_2$. There may be promising applications of the electric current-induced switchability of TiO$_2$ for memristor technology. 


\paragraph{Acknowledgements}

The authors would like to thank Bekki Mills and Elijah Stevens for help with the design and implementation of the new in-situ sample environment at the Spallation Neutron Source at Oak Ridge National Laboratory. Work at the University of Colorado was supported by U.S. Department of Energy, Office of Basic Energy Sciences, Office of Science, under Contract No. DE-SC0024117. Research at ORNL’s SNS was sponsored by the Scientific User Facilities Division, Office of Basic Energy Sciences, U.S. Department of Energy (DOE). T.S. was supported by the U.S. Department of Energy, Office of Science, Office of Workforce Development for Teachers and Scientists, Office of Science Graduate Student Research (SCGSR) program. The SCGSR program is administered by the Oak Ridge Institute for Science and Education for the DOE under contract number DE‐SC0014664. A.P., Y. Z., and G.C. acknowledge support by the National Science Foundation via Grant No. DMR 2204811.



\newpage
\section{SI}



\section{Determining the needle directions}

The directions of the diffuse scattering ``needles" are determined by fitting the coordinates of the intersection of the needles with integrated planes of intensity cut through the data. To improve statistics and remove the effects of structure factor on the intensity, we summed the data in all Brillouin zones with diffuse features into a single Brillouin zone. The fits are done using the intensity in the summed data sets. 

The original orientations of the needles were determined by fitting the intersections through planes perpendicular to the reciprocal lattice vectors of the crystal. These coordinates were used to construct projection vectors $\bm{u}$, $\bm{v}$, and $\bm{w}$, one set for each needle. The vectors are calculated in Cartesian coordinates with each vector having unit length, e.g. $|\bm{u}|=1~\textrm{\AA}^{-1}$. The vectors are chosen as follows: (i) $\bm{u}$ points along the needle and is found by fitting the intensity in cuts through the needle. (ii) $\bm{v}$ is chosen perpendicular to the plane containing the $\bm{u}$ vector of interest and a $\bm{u}$ vector belonging to a different needle. $\bm{w}$ is chosen as $\bm{w}=\bm{u}\times\bm{v}$. A set of projection vectors is shown in fig. S\ref{fig:uvw}. In the basis of a given needle, we specify coordinates $\bm{q}=\xi \bm{u} + \eta \bm{v} + \zeta \bm{w}$ where $\xi$, $\eta$, and $\zeta$ are the distance along $\bm{u}$, $\bm{v}$, and $\bm{w}$ respectively.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{flashed_rutile/uvw_fig.png}
    \caption{Projection vectors $\bm{u}$, $\bm{v}$, and $\bm{w}$ plotted with the summed S1 data set. $\bm{u}$ is parallel to the needle it is plotted on. $\bm{v}$ is in the plane containing two symmetry equivalent $\bm{u}$. $\bm{w}$ is parallel to $\bm{u}\times\bm{v}$.}
    \label{fig:uvw}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{flashed_rutile/rod_fit_figure.png}
    \caption{Fits to the needle directions in the S1 ((a),(b),(e)) and in-situ 100C, 500 mA ((c),(d),(f)) data sets. (a) Integrated data in the region shown in (e) taken from the summed S1 data set. (b) Fit to the data in (a). The coordinate of the intersection of the needle is $\bm{q}=\xi \bm{u} + \eta \bm{v} + \zeta \bm{w}$. For these cuts, $\xi=0.3$. In Cartesian coordinates, $\bm{q}=(0.06,0.21,0.20)~\textrm{\AA}^{-1}$. In reciprocal lattice units, $\bm{q}=(0.94,3.12,1.94)$. (c) Integrated data in the region shown in (f) taken from the in-situ 100C, 500 mA data set. (d) Fit to the data in (c). In Cartesian coordinates, the intersection is at $\bm{q}=(0.07,0.21,0.2)~\textrm{\AA}^{-1}$ and in reciprocal lattice units, $\bm{q}=(0.98,3.09,1.94)$.}
    \label{fig:needle_fits}
\end{figure}

Since the needles intersect planes perpendicular to the reciprocal lattice vectors at angles, the original integrated intensities are asymmetric, introducing error into the fits. To improve the fits, the original projections are used to integrate the data in planes that are approximately perpendicular to the needles. Planes are integrated in steps along each $\bm{u}$ vector and the coordinates of the needle are fit at each step. Examples of data integrated using the final projections are shown in fig. S\ref{fig:needle_fits} (a) and (c). In some cases, other needles than the one of interest in a given plane intersects near the origin too (see fig. S\ref{fig:needle_fits} (a)-(d)). To account for the other needles in a given plane, all of the needles intersecting each plane are fit simultaneously. The center, widths, and orientations of the intersections are denoted by the lines in fig. S\ref{fig:needle_fits} (b) and (d). The bold, unbroken lines correspond to the needle position of interest in each plane. The needle directions are all equivalent under tetragonal symmetry operations: the reported direction for each data set is determined by averaging the fits over all steps and over all needles. 


\begin{table}
\centering
\begin{tabular}{ | c | c c c | }
    \hline
    ~ & h & k & l \\
    \hline
    S1 & 1.00$\pm$0.02 & 3.08$\pm$0.02 & 1.93$\pm$0.01 \\ 
    100$^\circ$C 000mA & 1.01$\pm$0.02 & 3.00$\pm$0.02 & 2.00$\pm$0.02 \\
    100$^\circ$C 300mA & 0.97$\pm$0.04 & 3.01$\pm$0.04 & 2.02$\pm$0.03 \\
    100$^\circ$C 500mA & 1.01$\pm$0.05 & 3.06$\pm$0.05 & 1.93$\pm$0.03 \\
    400$^\circ$C 000mA & 1.02$\pm$0.05 & 2.94$\pm$0.05 & 2.03$\pm$0.02 \\ 
    400$^\circ$C 950mA & 1.01$\pm$0.04 & 3.00$\pm$0.05 & 1.99$\pm$0.02 \\ 
    \hline
    ~ & 1.00$\pm$0.04 & 3.02$\pm$0.04 & 1.98$\pm$0.02 \\
    \hline
    S2 & 0.99$\pm$0.02 & 3.02$\pm$0.04 & 1.99$\pm$0.05 \\
    \hline
\end{tabular}
\caption{Directions (in r.l.u.) of the (132) needles in the diffuse scattering. The needle direction for each data set is determined by fitting the intersection of the needle as discussed in the text. The reported values are averaged over all needles in each summed data set. The error bars are standard deviations. \label{table:needle_pos}}
\end{table}

The directions of the $k_1$ needle for all data sets are given in table \ref{table:needle_pos}. We call the needles $k_1$, $k_2$, ..., $h_1$, $h_2$, ... etc. The letter denotes which face of the Brillouin zone they intersect. The subscripts label the different needles as shown in fig. \ref{fig:needle_labels}. $k_1$ has all components positive. The other needles can be obtained by applying tetragonal symmetry operations.

For the (225) needles, quantitative analysis was more difficult since the intensity of the needles is weaker and decays more quickly away from the Bragg peak than the (132) needles. The (225) needles are only present in the S2 dataset, but were determined to point along (225) by fitting with same procedure described above. 

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{flashed_rutile/293K_quenched_summed_iso.jpg}
    \caption{Label of the different needles discussed in the text. The volumetric data are from the summed S1 dataset.}
    \label{fig:needle_labels}
\end{figure}


\section{Summed datasets}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/all_summed.png}
    \caption{Summed views of all datasets (see discussion in the text). The blue vectors show the direction of current; the red vectors label the scattering plane. In the ex-situ data, the \emph{dashed} blue vectors represent the direction current flowed during flash; no current was applied during the neutron scattering experiment.}
    \label{fig:all_summed}
\end{figure}

As discussed in the main text, qualitative analysis of the diffuse scattering data is frustrated by the structure factor: diffuse scattering around the Bragg peaks is asymmetric and varies from Brillouin zone to Brillouin zone. To aid in the analysis and visualization of the diffuse scattering, we picked all Brillouin zones showing significant diffuse scattering and summed them to a single Brillouin zone. Specifically, let $\bm{Q}=\bm{G}+\bm{q}$, with $\bm{G}$ a reciprocal lattice vector labeling an extended Brillouin zone and $\bm{q}$ a reduced wave vector. We selected all $\bm{G}$ with significant diffuse scattering and translated them to a single Brillouin zone, then summed the data at equivalent $\bm{q}$ in the chosen zones. The summed intensity for all datasets measured are presented in fig. S\ref{fig:all_summed}. 

In fig. S\ref{fig:all_summed}, the blue vectors show the direction of current; the red vectors label the scattering plane. In the in-situ data, the current was always in the scattering plane. In the ex-situ data, the sample was mounted different for different experiments. 

The fuzzy background in the in-situ datasets is scattering the furnace. The prominent diffuse scattering features are correlated with the size of the current; with increasing current, the sea-urchin like features enhance (see main text). 

The funny looking features, labeled as artifacts, are a nuance of the experiments. Bragg scattering is incredibly strong and saturated the entire detector tubes, resulting in curved rods perpendicular to the scattering planes. Examples of the artifacts in the raw (i.e. not summed) S1 and S2 datasets are shown at $\bm{Q}=(2,0,0)$ and $\bm{Q}=(2,1,0)$ in fig. S\ref{fig:funny_features}.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/funny_features_w_arrows.png}
    \caption{Volumetric plots of diffuse scattering in the $\bm{Q}=(2,0,0)$ and $\bm{Q}=(2,1,0)$ zones in the raw (i.e. not summed) S1 (current along $b$-axis) and S2 (current along $c$-axis) datasets. The funny features labeled in the figures originating from saturated detectors during the experiment.}
    \label{fig:funny_features}
\end{figure}

\section{Curie-Weiss fits to magnetic susceptibility}

In table \ref{table:CW_fits}, we provide the results of Curie-Weiss fits to the magnetic susceptibilities over the full and low temperature ranges as discussed in the main text.

\begin{table}
\centering
\begin{tabular}{ | c | c c c c | }
    \hline  
    ~ & $\chi^p_{ab}$ & $\chi^p_{c}$ & $\chi^f_{ab}$ & $\chi^f_{c}$  \\
    \hline
    $\mu_{eff}$ ($\mu_B$/Ti) & 0.024 & 0.025 & 0.069 & 0.065 \\
    (all T) & 0.035 & 0.061 & 0.092 & 0.087 \\
    \hline 
    $\theta_{cw}$ (K) & -2.2 & -3.2 & -0.9 & -0.7 \\
    (all T) & -7.1 & -25.6 & -3.8 & -3.6 \\
    \hline
    $\chi_0 \times 10^5$ (emu/mol/Oe) & 8.0 & 3.3 & 20.0 & 29.0 \\
    (all T) & 7.8 & 2.7 & 19.0 & 28.0 \\
    \hline
\end{tabular}
\caption{Results of fitting magnetic susceptibilities of pristine rutile TiO$_2$ along the $ab$ plane, $\chi^p_{ab}$, and along the $c$ axis, $\chi^p_{c}$ and the flashed S2 sample along the $ab$ plane, $\chi^f_{ab}$, and along the $c$ axis, $\chi^f_{c}$. We provide fits to the low-T regime (T$\leq$ 50 K) and all temperature (``all-T"). \label{table:CW_fits}}
\end{table}




\section{Integrating data along arbitrary projections}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{flashed_rutile/voxels.png}
    \caption{Overlapping integration bins voxels. The red regions correspond to the integration weights, i.e. the ``volume" of the overlap.}
    \label{fig:voxels}
\end{figure}

The diffuse scattering data lie on a 3-dimensional rectilinear grid. Each element is called a \emph{voxel}. To make 1-dimensional cuts along and perpendicular to the needles, we want to rehistogram the data. However, the needles do not point along a grid edge. \textsc{mantid} \cite{ARNOLD2014156} was used for data reduction and manipulation, but as of this writing, there are no algorithms in \textsc{mantid} for rehistogramming data in a direction that isn't commensurate with the voxels.

To rehistogram the data, we define a direction in which want to integrate and specify the bin spacing in each direction. We call the directions $\bm{u}$, $\bm{v}$, and $\bm{w}$ as discussed above. The combined set $\hat{R}=(\bm{u},\bm{v},\bm{w})$ is called a ``projection" and we label the projection by $\hat{R}$, the matrix that transforms from the rectilinear coordinates of the voxels to the projection axes. To make 1-dimesional cuts along $\bm{u}$ (``line cuts"), we rebin along $\bm{u}$ and integrate over $\bm{v}$ and $\bm{w}$. Each bin along $\bm{u}$ is a rectanglular prism and all of the voxels are rectangular prisms (see fig. S\ref{fig:voxels}). Each voxel that falls into a bin contributes some amount of weight. If the full voxel lies in a bin, its weight in that bin is 1. If it is partially in the bin, its weight is equal to the volume of overlap normalized by the total volume of the voxel. In the case that the binning projection is parallel to the voxel edges, calculating the weights is relatively easy. When the projection lies in an arbitrary direction, calculating the overlap between bins and voxels is mathematically straightforward but is computationally challenging. As a work around, we use an approximate strategy.  

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{flashed_rutile/butterworth.pdf}
    \caption{1-dimensional Butterworth function for several values of $n$, all with $\Delta q = 1$ and $q_0 = 0$. For small $n$, the edge of the bin is broad. For large $n$, the edge is sharp. $x_0 =0$ and $\Delta x = 1$. The bold, black line is a square pulse, showing the limit $n\rightarrow \infty$.}
    \label{fig:butterworth_1d}
\end{figure}

Let us restate the problem in words. Consider only a single bin from here on. We want to integrate around an interesting feature in the data to improve statistics and do further analysis. Let $\bm{q}_0$ be the coordinate of the feature in voxel coordinate system. We want voxels near the interesting feature (near the bin center) to contribute significantly to the integral, but voxels far away (near the bin edges) to contribute less. This is the same idea as in fig. S\ref{fig:voxels}. Voxels fully in the bin have weight 1, but voxels only partially in the bin have lower weight. To approximate this scheme, we define a weighting function, $w(\bm{q})$, that is 1 for voxels that are in the middle of a bin and decay to 0 near the edge of the bin. $\bm{q}$ are the coordinates of the center of the voxels. A good function for this is the ``Butterworth function". Its 1-dimensional version is 
\begin{equation}
    w(q) = \left[1+\left(\frac{q-q_0}{\frac{1}{2}\Delta q}\right)^n \right]^{-1} .
    \label{eq:butterworth_1d}
\end{equation}
$q_0$ specifies the bin center and $\Delta q$ is the bin width; it is the full-width at half-maximum (FWHM) of the Butterworth function. $n$ is an even integer that controls how quickly the functions decays from 1 to 0 near the edge of bin. In other words, it controls how much voxels near the bin edges contribute to the integral. The 1-dimensional Butterworth function is plotted for several $n$ in fig. S\ref{fig:butterworth_1d}.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/butterworth_2d.pdf}
    \caption{2-dimensional Butterworth function for several different widths and projections. The grid represents edges of voxels and the colormap shows the weight of each voxel in the bin; the bin edges are denoted by the dashed line. In the left panel, $\Delta x = \Delta y = 4$ and $x_0 = y_0 = 0$. In the middle, the center is shifted to $x_0 = y_0 = 1$ and the widths are $\Delta x = 4$, $\Delta y = 2$. The projection is still parallel to the voxel edges. In the right panel, the center and widths are the same as the middle but the projection is rotated by $45^\circ$ from the voxel axes.}
    \label{fig:butterworth_2d}
\end{figure}

The 3-dimensional generalization of the Butterworth function is 
\begin{equation}
    w(\bm{q}) = \left[\left(1+\left(\frac{h-h_0}{\frac{1}{2}\Delta h}\right)^n\right) \left(1+\left(\frac{k-k_0}{\frac{1}{2}\Delta k}\right)^n\right) \left(1+\left(\frac{l-l_0}{\frac{1}{2}\Delta l}\right)^n\right) \right]^{-1} .
    \label{eq:butterworth_3d}
\end{equation}
$h_0$, $k_0$, and $l_0$ are the $h$, $k$, and $l$ coordinates of the bin center in Cartesian coordinates. $\Delta h$, and $\Delta k$, and $\Delta l$ are the widths of the bins along the directions parallel to $h$, $k$, and $l$.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{flashed_rutile/293K_quenched_H2.73_K1.36_L1.36_u_cuts.pdf}
    \caption{Integration weights for a line cut along the $h_3$ needle (``along $\bm{u}$") at the $\bm{Q}=(2,1,2)$ Bragg point (fig. S\ref{fig:212}. Bins along the needle are $0.05 \textrm{\AA}^{-1}$ thick and are integrated $\pm 0.075 \textrm{\AA}^{-1}$ in the perpendicular direction.}
    \label{fig:212_u_cuts}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{flashed_rutile/293K_quenched_H2.73_K1.36_L1.36_v_cuts.pdf}
    \caption{Integration weights for a line cut perpendicular to the $h_3$ needle (``along $\bm{v}$") at the $\bm{Q}=(2,1,2)$ Bragg point (fig. S\ref{fig:212}. Bins along the needle are $0.05 \textrm{\AA}^{-1}$ thick and are integrated $\pm 0.075 \textrm{\AA}^{-1}$ in the perpendicular direction. The cut is offset from the Bragg peak by a distance $\xi=0.3 \textrm{\AA}^{-1}$ along $\bm{u}$.}
    \label{fig:212_v_cuts}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{flashed_rutile/293K_quenched_H2.73_K1.36_L1.36_w_cuts.pdf}
    \caption{Integration weights for a line cut perpendicular to the $h_3$ needle (``along $\bm{w}$") at the $\bm{Q}=(2,1,2)$ Bragg point (fig. S\ref{fig:212}. Bins along the needle are $0.05 \textrm{\AA}^{-1}$ thick and are integrated $\pm 0.075 \textrm{\AA}^{-1}$ in the perpendicular direction. The cut is offset from the Bragg peak by a distance $\xi=0.3 \textrm{\AA}^{-1}$ along $\bm{u}$.}
    \label{fig:212_w_cuts}
\end{figure}

To use the Butterworth function to rehistrogram, we define the coordinate of the bin center, $\bm{q}_0 = (h_0,k_0,l_0)^T$, the widths $\Delta \bm{q} = (\Delta h, \Delta k, \Delta l)^T$, and projection directions $\bm{u}$, $\bm{v}$, $\bm{w}$ based on the feature we are interested in. The widths are parallel to the projection axes. To integrate along a particular direction, we rotate the voxel coordinate system to be aligned with the projection directions. We assume the voxel coordinates are orthonormal so that the rotation matrix $\hat{R}=(\bm{u},\bm{v},\bm{w})$ is just the matrix of projection vectors. Since the rotation is around the origin, to integrate along a feature that is offset from the origin at position $\bm{q}_0$, we must first translate the center of the feature to the origin. Then $\bm{q}' = \hat{R}(\bm{q}-\bm{q}_0)$. We evaluate the Butterworth function for the new coordinates $\bm{q}'$, giving us the weights of the coordinates originally at $\bm{q}$ that fall in our bin centered on $\bm{q}_0$. 

We provide a 2-dimensional example of this approximate procedure to calculate weights in fig. S\ref{fig:butterworth_2d}.
The 2-dimensional version of the Butterworth is an obvious generalization of eq. S\ref{eq:butterworth_3d}. The weights are denoted by the colormap. Even in the case where the projection axes are rotated, the voxels at the edge of the bin indeed contribute less to the integration ($w < 1$) while voxels in the middle of the bin contribute most strongly ($w=1$). This is the desired outcome. 

The data in fig. S\ref{fig:needle_fits} are integrated using this scheme; the weights calculated by the Butterworth function are shown in fig. S\ref{fig:needle_fits} e) and f). As another example, we plot the integration weights for the line cuts along the $h_3$ needle at the $\bm{Q}=(2,1,2)$ in fig. S\ref{fig:212_u_cuts} and for the line cuts perpendicular to the $\bm{Q}=(2,1,2)$ $h_3$ needle in figs. S\ref{fig:212_v_cuts} and S\ref{fig:212_w_cuts}.

We used method described here, with $n=40$, for all line cuts in this supplementary document and in the main text.

\section{Resolution}

\begin{table}
\centering
\begin{tabular}{ | c | c c c c  c c c c | }
    \hline
    $\textrm{\AA}^{-1}$ & $k_1$ & $k_2$ & $k_3$ & $k_4$ & $h_1$ & $h_2$ & $h_3$ & $h_4$ \\
    \hline
    $\sigma$ & 0.0762 & 0.0762 & 0.0778 & 0.0769 & 0.0569 & 0.0582 & 0.0545 & 0.0543 \\
    \hline
\end{tabular}
\caption{Experimental resolution in the direction of each needle determined by fitting line cuts through diffuse scattering from a pristine TiO$_2$ crystal. The results, $\sigma$, are FWHM of Gaussians, in $\textrm{\AA}^{-1}$, fit to the data. \label{table:resolution}}
\end{table}

The experimental resolution is estimated by fitting the diffraction data from a pristine crystal under the same experimental conditions as the S1 data sets (i.e. room temperature with out a furnace and the same crystal orientation). Pristine data are plotted alongside S1 data in figs. S\ref{fig:002}, S\ref{fig:202},  S\ref{fig:212},  S\ref{fig:301},  S\ref{fig:310}, and S\ref{fig:410}. We attempted to fit the pristine data with Voight functions; however, the result was vanishing Lorentzian component. The Bragg peaks in the pristine data are best described by pure Gaussians. The resolution is anisotropic, so it is useful to estimate it along the direction of each needle. We fit line cuts in the direction of each needled through multiple pristine Bragg peaks and averaged over the Bragg peaks. The results characterizing the resolution are presented in table \ref{table:resolution}.

\section{Line cuts through the diffuse scattering}

To show the asymmetry of the diffuse scattering around Bragg peaks and to show structure factor of the diffuse scattering, we pick a handful of symmetry-inequivalent Bragg points and plot line cuts along each needle in the S1 data set. Figs. S\ref{fig:002}, S\ref{fig:202},  S\ref{fig:212},  S\ref{fig:301},  S\ref{fig:310}, and S\ref{fig:410} show the data at the select points. Interestingly, even though the electric field in the $ab$ plane breaks the tetragonal symmetry, the data still exhibit tetragonal symmetry within numerical error. To improve statistics, all line cuts that are equivalent under $Pmmm$ symmetry are averaged.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/quenched_cuts_H0.00_K0.00_L2.00.pdf}
    \caption{Line cuts along the diffuse scattering needles at the $\bm{Q}=(0,0,2)$ point in the S1 data set. The data are integrated $0.05 \textrm{\AA}^{-1}$ along the cut and $\pm 0.075 \textrm{\AA}^{-1}$ perpendicular to the cut. The volumetric plot of the data in this zone labels the needles. The solid black line with circular markers is diffuse scattering from the S1 crystal; the broken magenta line is scattering from a pristine crystal.}
    \label{fig:002}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/quenched_cuts_H2.00_K0.00_L2.00.pdf}
    \caption{Line cuts along the diffuse scattering needles at the $\bm{Q}=(2,0,2)$ point in the S1 data set. The binning and legend is the same as fig. S\ref{fig:002}.}
    \label{fig:202}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/quenched_cuts_H2.00_K1.00_L2.00.pdf}
    \caption{Line cuts along the diffuse scattering needles at the $\bm{Q}=(2,1,2)$ point in the S1 data set. The binning and legend is the same as fig. S\ref{fig:002}.}
    \label{fig:212}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/quenched_cuts_H3.00_K0.00_L1.00.pdf}
    \caption{Line cuts along the diffuse scattering needles at the $\bm{Q}=(3,0,1)$ point in the S1 data set. The binning and legend is the same as fig. S\ref{fig:002}.}
    \label{fig:301}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/quenched_cuts_H3.00_K1.00_L0.00.pdf}
    \caption{Line cuts along the diffuse scattering needles at the $\bm{Q}=(3,1,0)$ point in the S1 data set. The binning and legend is the same as fig. S\ref{fig:002}.}
    \label{fig:310}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/quenched_cuts_H4.00_K1.00_L0.00.pdf}
    \caption{Line cuts along the diffuse scattering needles at the $\bm{Q}=(4,1,0)$ point in the S1 data set. The binning and legend is the same as fig. S\ref{fig:002}.}
    \label{fig:410}
\end{figure}
\begin{figure}
    \includegraphics[width=1\linewidth]{flashed_rutile/quenched_vw_cuts.pdf}
    \caption{Cuts perpendicular to the diffuse scattering needles near the Bragg peaks at $\bm{Q}=(3,1,0)$ a)-d), $\bm{Q}=(2,1,2)$ e)-h), and $\bm{Q}=(2,0,2)$ i)-l). a), c), e), g), i), and k) are parallel to $\bm{v}$ and b), d), f), h), j), and l) are parallel to $\bm{w}$; $\bm{v}$ and $\bm{w}$ are mutually orthogonal vectors perpendicular to the needle. Which needle is labeled in each panel.}
    \label{fig:vw_cuts_2}
\end{figure}

Needles in reciprocal space correspond to pancake-like correlations in real space. Fitting the needles tells us the size of the correlated regions in real space: specifically, the decay length of the diffuse scattering is reciprocal to the size of the correlations in real space. For pancake-like correlations, the decay length along the needle describes the correlation length between defect planes and the decay length perpendicular to the needles describes the size of the correlations in the planes.

Along the needles, diffuse scattering tails were fit with a Voight function with Lorentzian full-width at half-maximum (FWHM) $\Gamma_\parallel$ and Gaussian standard deviation $\sigma_\parallel$. The Lorentzian component corresponds to the correlations, with the Gaussian part corresponding to resolution broadening. Near each Bragg peak, multiple needles intersect and the fit along a particular needle in this region isn't meaningful. We accounted for the intersection of multiple needles at the Bragg peak by adding an additional Gaussian with standard deviation $\sigma_B$. The width and amplitude of the Gaussian at the Bragg peak was the same for all needles at a given peak: i.e. all needles intersecting a given Bragg peak were fit simultaneously. The background was approximated by constant offset, $s$. All reciprocal lengths have units $\textrm{\AA}^{-1}$. Because the structure factor is asymmetric, each side of the peak was fit separately. 

The results of fitting the line cuts through the S1 data along the needles are shown in figs. S\ref{fig:310_k1_fits}, S\ref{fig:310_k2_fits}, S\ref{fig:212_h3_fits}, S\ref{fig:212_h4_fits}, S\ref{fig:202_k2_fits}, and S\ref{fig:202_k4_fits}. Averaging over all Lorentzian fits, we estimate the correlation length perpendicular to the defects to be 46.62 $\textrm{\AA}$.

We also made line cuts perpendicular to the needles to show the width. These are shown in figs. S\ref{fig:vw_cuts_1} and S\ref{fig:vw_cuts_2} for select Bragg peaks. To estimate the size of the pancake-like defects, we fit the widths of the needles. Since multiple needles intersect near the Bragg peaks, the fits near the Bragg peaks aren't meaningful. We focused on the needles sufficiently far from the Bragg peaks to avoid spurious fits, but the signal to background ratio is poor and the fits were difficult. To make the fits as simple as possible, we assumed a pure Lorentzian. The results of fitting cuts perpendicular to the needles are shown in figs. S\ref{fig:310_vw_fits}, S\ref{fig:212_vw_fits}, and S\ref{fig:202_vw_fits}. 
 
The different curves correspond to cuts at different distances from the Bragg peaks. $\Gamma_\perp$ is the FWHM of the Lorentzian fit perpendicular to the needle. The fits vary from 0.0004 $\textrm{\AA}^{-1}$ to 0.0142 $\textrm{\AA}^{-1}$ (two orders of magnitude) depending on how close to the Bragg peaks and along which direction we look. These fits are resolution limited and large variation in the fitting frustrates the interpretation. Moreover, neglecting the Gaussian part of the Voight forces the Lorentzian width to be overestimated. Still, if we assume a representative width of 0.005 $\textrm{\AA}^{-1}$, then the sizes of the defects in real space are approximately $\sim 200$ $\textrm{\AA}$.


\begin{figure}
    \includegraphics[width=\linewidth]{flashed_rutile/quenched_vw_cuts.pdf}
    \caption{Cuts perpendicular to the diffuse scattering needles near the Bragg peaks at $\bm{Q}=(3,1,0)$ a)-d), $\bm{Q}=(2,1,2)$ e)-h), and $\bm{Q}=(2,0,2)$ i)-l). a), c), e), g), i), and k) are parallel to $\bm{v}$ and b), d), f), h), j), and l) are parallel to $\bm{w}$; $\bm{v}$ and $\bm{w}$ are mutually orthogonal vectors perpendicular to the needle. Which needle is labeled in each panel.}
    \label{fig:vw_cuts_1}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{flashed_rutile/fits_Q_3_1_0_k1.pdf}
    \caption{Results of fitting the length of the $k_1$ needle at the $\bm{Q}=(3,1,0)$ Bragg peak. The tails were fit with a Voight function with Lorentzian FWHM $\Gamma_\parallel$ and Gaussian standard deviation $\sigma_\parallel$. The intersection of all needles at the center of the Bragg peak was approximated by Gaussian with standard deviation $\sigma_B$. The background was approximated by constant offset, $s$. Because the structure factor is asymmetric, each side of the peak was fit separately. All quantities have units $\textrm{\AA}^{-1}$.}
    \label{fig:310_k1_fits}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{flashed_rutile/fits_Q_3_1_0_k2.pdf}
    \caption{Results of fitting length of the $k_2$ needle at the $\bm{Q}=(3,1,0)$ Bragg peak. The description is the same as fig. S\ref{fig:310_k1_fits}.}
    \label{fig:310_k2_fits}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{flashed_rutile/fits_Q_2_1_2_h3.pdf}
    \caption{Results of fitting length of the $h_3$ needle at the $\bm{Q}=(2,1,2)$ Bragg peak. The description is the same as fig. S\ref{fig:310_k1_fits}.}
    \label{fig:212_h3_fits}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{flashed_rutile/fits_Q_2_1_2_h4.pdf}
    \caption{Results of fitting length of the $h_4$ needle at the $\bm{Q}=(2,1,2)$ Bragg peak. The description is the same as fig. S\ref{fig:310_k1_fits}.}
    \label{fig:212_h4_fits}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{flashed_rutile/fits_Q_2_0_2_k2.pdf}
    \caption{Results of fitting length of the $k_2$ needle at the $\bm{Q}=(2,0,2)$ Bragg peak. The description is the same as fig. S\ref{fig:310_k1_fits}.}
    \label{fig:202_k2_fits}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{flashed_rutile/fits_Q_2_0_2_k4.pdf}
    \caption{Results of fitting length of the $k_4$ needle at the $\bm{Q}=(2,0,2)$ Bragg peak. The description is the same as fig. S\ref{fig:310_k1_fits}.}
    \label{fig:202_k4_fits}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{flashed_rutile/quenched_vw_fits_Q_3_1_0.pdf}
    \caption{Result of fitting the width of the $k_1$ (a,b) and $k_2$ (c,d) needles at the $\bm{Q}=(3,1,0)$ Bragg peak. $\Gamma_\perp$ is the Lorentzian FWHM of the width of the needle in $\textrm{\AA}^{-1}$. a) and c) are along $\bm{v}$ and b) and d) are along $\bm{w}$. $\xi$ is distance ($\textrm{\AA}^{-1}$) along $\bm{u}$ from the Bragg peak (see figs. S\ref{fig:212_v_cuts} and S\ref{fig:212_w_cuts}).}
    \label{fig:310_vw_fits}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{flashed_rutile/quenched_vw_fits_Q_2_1_2.pdf}
    \caption{Result of fitting the width of the $h_3$ (a,b) and $h_4$ (c,d) needles at the $\bm{Q}=(2,1,2)$ Bragg peak. $\Gamma_\perp$ is the Lorentzian FWHM of the width of the needle in $\textrm{\AA}^{-1}$. a) and c) are along $\bm{v}$ and b) and d) are along $\bm{w}$. $\xi$ is distance ($\textrm{\AA}^{-1}$) along $\bm{u}$ from the Bragg peak (see figs. S\ref{fig:212_v_cuts} and S\ref{fig:212_w_cuts}).}
    \label{fig:212_vw_fits}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{flashed_rutile/quenched_vw_fits_Q_2_0_2.pdf}
    \caption{Result of fitting the width of the $k_2$ (a,b) and $k_4$ (c,d) needles at the $\bm{Q}=(2,0,2)$ Bragg peak. $\Gamma_\perp$ is the Lorentzian FWHM of the width of the needle in $\textrm{\AA}^{-1}$. a) and c) are along $\bm{v}$ and b) and d) are along $\bm{w}$. $\xi$ is distance ($\textrm{\AA}^{-1}$) along $\bm{u}$ from the Bragg peak (see figs. S\ref{fig:212_v_cuts} and S\ref{fig:212_w_cuts}).}
    \label{fig:202_vw_fits}
\end{figure}


\section{Momentum dependence of diffuse scattering}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/quenched_vs_K.pdf}
    \caption{$\bm{Q}$-dependence, for integer $K=1$ rlu, of diffuse scattering from the ex-situ S1 dataset, with current along $\bm{k}$. The dark regions show pronounced diffuse scattering.}
    \label{fig:K_dep_quenched}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/quenched_vs_K_near_1.pdf}
    \caption{$\bm{Q}$-dependence near $K=1$ of diffuse scattering from the ex-situ S1 dataset, with current along $\bm{k}$. The dark regions show pronounced diffuse scattering.}
    \label{fig:K_dep_quenched_near_1}
\end{figure}


We show colormaps of the diffuse scattering in the S1 dataset for several $K$ values. Fig. S\ref{fig:K_dep_quenched} shows diffuse scattering at integer $K$ values, showing how the structure factor evolves in reciprocal space. Fig. S\ref{fig:K_dep_quenched_near_1} shows several $K$ values around $K=1$ (rlu), showing how the diffuse scattering needles disperse near Bragg peaks. 


\section{Current dependence of diffuse scattering}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{flashed_rutile/current_dep.pdf}
    \caption{$\bm{Q}$-dependence near $K=1$ of diffuse scattering from the ex-situ S1 dataset, with current along $\bm{k}$. The dark regions show pronounced diffuse scattering.}
    \label{fig:current_dep}
\end{figure}

Line cuts along the diffuse scattering needles at several select Bragg peaks for several current densities are presented in the main text. In fig. S\ref{fig:current_dep}, we show color maps of the same datasets across a larger region of reciprocal space. 

